Fock-Goncharov coordinates for rank two Lie groups

Let G be a simply connected, simple, complex Lie group of rank 2. We give explicit Fock-Goncharov coordinates for configurations of triples and quadruples of affine flags in G. We show that the action on triples by orientation preserving permutations corresponds to explicit quiver mutations, and that the same holds for the flip (changing the diagonal in a quadrilateral). This gives explicit coordinates on higher Teichmuller space, and also coordinates for boundary-unipotent representations of 3-manifold groups. As an application, we compute the (generic) boundary-unipotent representations in Sp(4,C) for the figure-eight knot complement.

==> figures_gen/QB213.tex <==
\begingroup
 \setlength{\unitlength}{0.8pt}
 \begin{picture}(291.42392,288.00842)
 \put(0,0){\includegraphics{figures_gen/QB213_included}}
 \end{picture}
\endgroup

